Towards Deploying a Scalable & Robust Vehicular Identity and Credential Management Infrastructure

Several years of academic and industrial research efforts have converged to a common understanding on fundamental security building blocks for the upcoming Vehicular Communication (VC) systems. There is a growing consensus towards deploying a Vehicular Public-Key Infrastructure (VPKI) enables pseudonymous authentication, with standardization efforts in that direction. However, there are still significant technical issues that remain unresolved. Existing proposals for instantiating the VPKI either need additional detailed specifications or enhanced security and privacy features. Equally important, there is limited experimental work that establishes the VPKI efficiency and scalability. In this paper, we are concerned with exactly these issues. We leverage the common VPKI approach and contribute an enhanced system with precisely defined, novel features that improve its resilience and the user privacy protection. In particular, we depart from the common assumption that the VPKI entities are fully trusted and we improve user privacy in the face of an honest-but-curious security infrastructure. Moreover, we fully implement our VPKI, in a standard-compliant manner, and we perform an extensive evaluation. Along with stronger protection and richer functionality, our system achieves very significant performance improvement over prior systems - contributing the most advanced VPKI towards deployment.

==> system-adversary-model.tex <==
\section{Adversary Model}
\label{sec:system-adversary-models}



%In a \ac{VC} system, \textit{faulty} nodes or adversaries are categorized into \textit{internal} and \textit{external} \cite{papadimitratos2006securing}. \textit{Internal} adversaries are the legitimate entities within the system, provided with credentials (long-term and pseudonym certificates). They might participate in performing attacks intentionally or unintentionally. On the contrary, \textit{external} adversaries exploit the system without being part of it since they are not equipped with valid credentials. They might try to make some faked requests to the infrastructure entities to endanger the availability of the system. We do not consider internal adversaries in our scheme since the compromising vehicles are evicted from the system in case of deviation from the \ac{VC} system policies or protocols. 

Our security and privacy requirements comply with the comprehensive security and privacy requirements for \acp{VANET}, as discussed in \cite{papadimitratos2006securing}. Additionally, we consider the behavior of infrastructure side entities from two perspectives: 

%, with the help of collaborating users,
\begin{itemize}
	\item \textit{Honest-but-curious Authorities:} Infrastructure entities are considered honest, but not fully-trusted; they might try to infer information from clients in order to profile users. In other words, authorities might be curious to link users to predict their behaviors and subsequently, benefit from them.
	% An example is to track users and see which places they are visiting and as a result, they can advertise to those users, who visited that places. 

	\item \textit{Colluding Authorities:} The infrastructure entities might collude to deduce some information and thus, infringing the users privacy.  

%	\item \textit{Byzantine or Malicious Authorities:} \acp{PCA} might misbehave in issuing pseudonyms while at the same time the \ac{LTCA} might misbehave in authenticating users. Moreover, \ac{RA} might also misbehave in resolving or revoking the pseudonyms. 
	
%	\item \textit{External \ac{GPA}:} He eavesdrops the messages in order to violate users' privacy by linking the pseudonyms. 
	%In case an entity misbehaves, the corresponding authorities can identify it through the resolution process, as discussed in security analysis in Sec. \ref{sec:security-analysis}. 
\end{itemize}

%There is no misbehavior detection authority in our scheme in order to detect and report the misbehaving entities to the \ac{RA}. Moreover, 

%We consider an external \ac{GPA}, who eavesdrops the messages in order to violate users' privacy by linking the pseudonyms. 

%Our adversarial model consists of an external \ac{GPA}, eavesdropping the messages in order to violate users' privacy by linking the pseudonyms. 

%However, jamming and \ac{DDoS} are beyond the scope of our paper. % and we do not discuss them. 



%we consider what the infrastructure does possibly with the help of collaborating users

%Whereas \textit{external} adversaries are not the legitimate part of the system and as a result, they are not equipped with credentials. 

%\textit{Input-controlling} in a system with secure credential management scheme is feasible since vehicles might be able to feed the protocol input with faked data. This yields in consuming infrastructure resources while not deviating from system security protocols. However, they might In this way, they would manage to perform other attacks like \ac{DoS}. As an example, if an adversary sends a pseudonym request to \ac{PCA} with incorrect signature on the message, she would manage to leech server resources. %However, they can still carry some attacks like: replay messages, selective DoS, etc \cite{papadimitratos2006securing}. 

%Performing a \textit{Sybil} attack \cite{douceur2002sybil} is feasible if vehicles are able to  In other words, 

%Based on \cite{papadimitratos2006securing}, the adversary model is ... 

%There is no strong assumption on trust relationship among infrastructure entities since in our system, \ac{LTCA}, \ac{PCA} and \ac{RA} are not fully trusted. They might be \textit{curious} or \textit{malicious}; 

%A limited portion of entities might \textit{collude}. However, we assume that there is no collusion among all the entities at the same time. Obviously, if all the \acp{LTCA} and \acp{PCA} collude, the privacy of users is completely at stake. Furthermore, 
%However, in order to preform our experiments, we emulate the behavior of the misbehavior detection entity to accomplish our experiments. 


%Additional details are discussed in Sec. \ref{sec:security-analysis}, the security analysis.

%Who is the trusted entity in our system, who can tell lie and who cannot

%Linking attack between identity-Pseudonym 

%\textbf{R3. Honest-but-curious Entities:} 



%In \cite{wiedersheim2010privacy}, simple pseudonyms change is not enough 

% Service providers We do not assume any strong 

%***************************************
%\subsection{Assumptions}
%\label{subsec:assumptions}

%We assume that there are multiple domains, where vehicles can obtain services from any of them, depending on the policies. A domain is an area regulated under the same administrative policy; it can be a county, city or a country while it comprises many regions. In each domain, there are a few \acp{LTCA} while there exist several \acp{PCA}, where each of them is located in a region. Each vehicle is registered to one \ac{LTCA} while it can obtain services from any legitimate \ac{SP}, based on the policies and agreements. 



%We can assume that \acp{LTCA} are governmental agencies, which issue \acp{LTC} to the citizens while \acp{PCA} are independent private corporates. Additionally, each authority has a unique identifier which distinguishes itself from others. 

%In our system, \ac{LTCA}, \ac{PCA} and \ac{RA} are not fully trusted. 
%Infrastructure entities are referred as \acp{SIS}. 

%Vehicles are registered to their home \ac{LTCA} and authenticated to them while they choose their \acp{SP}. 


 %Partial collusion among the entities is considered safe if the infrastructure side entities have no prior knowledge on 




%Mention that there is no misbehavior detection now, since we are working on it. We assume that the corresponding entities figure out the misbehaving entities!!!!!


%We do not assume any hardware security module (HSM) to store credential


%In this paper, two different approaches in order to avoid multiple usages of a ticket is considered. In the \textit{indirect} approach, the back-end servers (\acp{PCA}) are communicating with each other in order to verify if the ticket has been obtained the appropriate service from another server. On the other hand, in the \textit{direct} mode, a ticket is verified by any \ac{SP} server \textit{locally} without communicating with other servers. 

\begin{comment}
%***************************************
\subsection{Security \& Privacy Requirements}
\label{subsec:security-privacy-requirements}

A \ac{VC} system comprises a huge amount of entities, including vehicles, mobile devices, users and infrastructure entities, e.g. \ac{RSU} and authorities. In such a heterogeneous and highly complex system, managing trust and identity is considered a difficult task. Vehicles from different manufacturers communicate with each other to disseminate warnings and traffic information. Considering the variety of such a ecosystem, all the aspects of security - from the three pillars of \ac{CIA}, to users' privacy - should be taken into account. Comprehensive security and privacy requirements for \acp{VANET} are discussed in \cite{papadimitratos2006securing}. In the following, the security requirements for a privacy-preserving identity and credential management scheme for \acp{VANET} are elaborated. 

%They are categorized into two sections; first, we address the general security requirements and afterwards, the design principles are explained. 

%The aim is to design the system, considering security and privacy requirements before deploying the system. Build-in and not add-on

%In a system, where each device is smart, equipped with appropriate hardware and software, it can communicate with other entities. 


%The security requirements are not limited to what have been discussed. There are some other requirements, highly dependent to the system and affects on it, such as: 

%\textit{Honest-but-curious} authorities 


%We have devices talks with device, we have device talk to the control systems, to ITS, to back end systems, which of course requires many requirements such as highly inter connected systems and network 

%Users in smart cities are supposed to be ensured about their privacy in order to participate in the services, provided in the system. Otherwise, they would never participate in the system and the users are sort of excluded by the system security policy and the non-privacy friendly protocols. 

%\textbf{R2. Non-repudiation}

%\textbf{R3. Entity Authentication} 


\textbf{R1. Message Authentication and Integrity:} The communication among vehicles and authorities is authenticated and prevented from alteration. 

\textbf{R2. Access Control:} Having authenticated the vehicles, a subset of the system is authorized and accessible according to the system policy.

\textbf{R3. Confidentiality:} The content of \ac{V2I} communication is kept secret from other entities. 

%so that the credentials cannot be used by others or linked???!!!!M!!!!. 

\textbf{R4. Privacy and Anonymity:} Users' privacy is protected to the full extent. Vehicles are communicating with each other anonymously while no single entity should be able to track or profile them. According to the \ac{VC} system security requirements \cite{raya2007securing}, the privacy of all the legitimate entities are protected as long as they do not deviate from the system security protocols and policies. Thus, the \ac{VPKI} does not provide full anonymity for the users due to liability purposes. 


\textbf{R5. Non-repudiation:} Every message is signed with the corresponding pseudonym private key in order to prevent clients from denying message transmission. 


\textbf{R6. Accountability and Liability Identification:} Every entity is legally responsible for all the activities during its life-time. Not only an entity cannot deny the activities he has done, but also he is liable and responsible for all of his commitments. 

\textbf{R7. Availability:} The system is available to offer services to the legitimate users and devices. Since \ac{VPKI} is considered a critical asset of the \ac{VC} system, compromising its availability could highly affect the human safety. 


\textbf{R8. Sybil-resilience:} A client cannot be equipped with multiple valid pseudonymous identities at the same time, even in multi-domain scheme with multiple \acp{PCA}. 

\textbf{R9. Perfect Forward Secrecy/Privacy:} All the communication remains confidential, even if the \acp{LTC} of the two-end communications are compromised. Moreover, perfect forward privacy implies that having resolved a pseudonym, no information should be revealed to infringe the privacy of the user in terms of linkability of the provided services, related credentials, etc.\cite{schaub2009privacy}. \textit{Escrow-foliage} should be supported to protect users privacy to the full extent. \textit{Escrow-foliage} states that the confidentiality and the privacy of the users' credentials should not be disclosed even if a completely trusted organization enforces the communication two end-points to reveal their long-term credentials. 


\textbf{R10. Revocation:} Misbehaving vehicles are entitled to be evicted form the system. Having identified the misbehaving vehicles, they cannot obtain pseudonyms from any \ac{PCA}. 


\end{comment}
%Privacy, unlinkability, conditional anonymity, 

%{\color{blue} Protecting users' and devices' privacy in such a ecosystem is considered challenging. On the one hand, entities are required to be authenticated and authorized; on the other hand, entities want to be anonymous in their everyday life (referred to as conditional anonymity\footnote{According to the \ac{VC} system security requirements, the privacy of all the legitimate entities are protected as long as they do not deviate from the system security protocols and policies. Thus, the \ac{VPKI} does not provide full anonymity for the users while it supports conditional anonymity.}). It is trivial that if users know that they are being monitored by \textit{``trusted authorities''}, they would be unwilling to participate in the system. In order to protect users' privacy, confidentiality of their identities, anonymity of their behavior, and unlinkability of their activities are needed to be protected.}

%Thus, short-term and long-term linkability to identify users and services are considered critical???.

%They want to be ensured about their privacy. 

%\textit{Smart City} communication system should never disclose, interpret or allow interference on the data communication. 

%Protecting users' privacy from the system and preventing system's inferences from the user are the main aim on this requirement. Devices are not supposed to be linkability on all of the activities they have done. Perfect forward privacy is required as well. 
%The privacy aspect of smart-cities should be taken into account by using the technologies, proposed in other domains
%What about Perfect Forward Privacy?
%Short-term and Long-term linkability? Short-term linkability identifies linkability in the short period of time while the long-term indicates in the long run. Pseudonyms are from the same sender while the other one is each pseudonym belongs to a specific driver name, or license plate number. Discussion on the road condition and road maps in order to prevent short-term linkability, is out side the scope of this paper as discussed in \cite{wiedersheim2010privacy}.

%Traceability

%The three pillar of privacy, confidentiality, anonymity and unlinkability, should be achieved by the system. 

%Having achieved the mentioned points, the unlinkability of the users, their requested services as well as the time of operations for each service would be achieved. 

%Prevention of vehicles to pretend to be multiple identities is critical since it can highly affect on the system safety, performance and transaction correctness. In some of the applications, the \acp{SP} rely on the data originated from the client side, illustrating the same incident. Therefore, Sybil-behaved entities might mislead the entire networks towards their goals. %The system should be resilient against Sybil behavior.

%When it comes to decision for benign vehicles, if they have received stuff from many different vehicles, specifically misbehavior detection, it .....  

%In the next section, the design principles are addressed. 


\begin{comment}
\subsection{Design Principles}
\label{subsec:design-principles}

\cite{papadimitratos2006securing} has proposed twelve design principles in order to safeguard the \ac{VC} systems against adversarial behavior. In the following, the design principles, applicable to the identity and credential management system for \acp{VANET}, are addressed. 

%\textbf{P9. Safety:} Since 

\textbf{P1. Efficiency \& Performance:} Considering the low latency requirement of safety applications in \ac{ITS}, the system should be highly-responsive. The performance of cryptographic operations are required to be efficient in order to react in a real-time manner. 

\textbf{P2. Separation of Privileges and Duties:} In order to diminish the risk of collusion among the infrastructure entities, the roles of them are split into multiple authorities. 
%In this way, users' privacy is 
%are required in order to split the roles and power in the system, so that diminishes the risk of collusion in order to infringe users' privacy.

%Splitting of the roles and power into 3 categiries of authorties, (LTCAs, PCAs and RAs) would 

\textbf{P3. Scalability:} The deployment of \ac{ITS} is expected to expand gradually (e.g., from big cities to countries), which implicates the need of a scalable system.

\textbf{P4. Resilience and Reliability:} The system is required to be able to withstand certain types of attacks and failures, while it does not affect the users' experiences.

\textbf{P5. Unique Identity:} A user, equipped with an unique identification, have a unified access method for different services. Using a unique identification and a unified access method, rather than multiple identifications for different services, can increase the utilization and accelerate the deployment of \ac{VC} systems.

%\textbf{P15. Internet connectivity:} In smart cities, different Internet connection methods are available for user (e.g., LTE for smart-phones and IEEE 802.11p for vehicles), thus increasing the accessibility of services. However, the heterogeneity of the network also motivates a need of a unified communication protocol.

\textbf{P6. Reconfigurability:} The proposed system should be easily reconfigurable in order to support interaction among vehicles from different manufacturers and domains. 

\textbf{P7. Privacy Conservation:} Based on the \textit{principle of psychological acceptability} \cite{matt2006introduction}, users' privacy should be protected as if no security mechanisms are present since users want to achieve at least the same level of privacy they have. 

\textbf{P8. Usability:} Not only from privacy conservation perspective, but also from usability viewpoint, the system should be simple and easy to use. Participation of the vehicles into the \ac{VC} system should be completely transparent to the users. 

\end{comment}


%\textbf{P9. Distributed Communication:} 
%V2V (Vehicle-2-Vehicle) and Peer-2-Peer


%\textbf{P9. Backward Compatibility:} The proposed \ac{VPKI} system should consider the integration of old vehicles into the system. In other words, integration of the vehicles, connected rarely to the network to obtain credentials, should be taken into account. 

%The pervasion of smart city technologies should happen transparently, thus ease of use is a key of popularizing smart city technologies. The lifestyle of users should not be changed significantly with utilization of such technologies.

%\textbf{R11. Governance:} 

%system and the users are sort of excluded by the system security policy and the non-privacy friendly protocols. 
 
%\textbf{P9. Contingency Plan and Disaster Recovery:} back up, etc.

%\textbf{P10. Data Storage Policies/Techniques:} Big data storage 



